Visual News: Benchmark and Challenges in News Image Captioning

We propose Visual News Captioner, an entity-aware model for the task of news image captioning. We also introduce Visual News, a large-scale benchmark consisting of more than one million news images along with associated news articles, image captions, author information, and other metadata. Unlike the standard image captioning task, news images depict situations where people, locations, and events are of paramount importance. Our proposed method can effectively combine visual and textual features to generate captions with richer information such as events and entities. More specifically, built upon the Transformer architecture, our model is further equipped with novel multi-modal feature fusion techniques and attention mechanisms, which are designed to generate named entities more accurately. Our method utilizes much fewer parameters while achieving slightly better prediction results than competing methods. Our larger and more diverse Visual News dataset further highlights the remaining challenges in captioning news images.

==> sections/Related_Work.tex <==
Image captioning has gained increased attention, with remarkable results in recent benchmarks. A popular paradigm~\cite{vinyals2015show, karpathy2015deep, donahue2015long} uses a convolutional neural network as the image encoder and generates captions using a recurrent neural network (RNN) as the decoder. The seminal work of~\citet{xu2015show} proposed to attend to different image patches at different time steps and~\citet{lu2017knowing} improved this attention mechanism by adding an option to sometimes not to attend to any image regions. Other extensions include attending to semantic concept proposals~\cite{you2016image}, imposing local representations at the object level~\cite{li2017image} and a bottom-up and top-down attention mechanism to combine object and other salient image regions~\cite{anderson2018bottom}.

News image captioning is a challenging task because the captions often contain named entities. Prior work has attempted this task by drawing contextual information from the accompanying articles. \citet{tariq2016context} select the most representative sentence from the article; \citet{ramisa2017breakingnews} encode news articles using pre-trained word embeddings and concatenate them with CNN visual features to feed into an LSTM~\cite{HochSchm97}; \citet{lu2018entity} propose a template-based method in order to reduce the vocabulary size and then later retrieves named entities from auxiliary data; \citet{biten2019good} also adopt a template-based method but extract named entities by attending to sentences from the associated articles. \citet{zhao-etal-2019-informative} also tries to generate more informative image captions by integrating external knowledge. \citet{tran2020transform} proposes a transformer method to generates captions for images embedded in news articles in an end-to-end manner. 
In this work, we propose a novel Transformer based model to enable more efficient end-to-end news image captioning.

\begin{figure}[t]
    \centering
      \includegraphics[width=0.43\textwidth]{sections/entity_s.pdf}
     %\vspace{-3pt}
    \caption{
    Average count of named entities per caption. We select the top 4 most frequent named entity types in our Visual News dataset. For example, in The Guardian, there are on average $0.72$ PERSON entities per caption while it is $0.46$ for BBC. We see that each agency employs a distinct captioning style.
    }
    \vspace{-0.2in}
    \label{fig:diversity_analysis1}
\end{figure}

\begin{table}[t]
\centering
\small
\begin{tabular}{ccccc}
\toprule
 & Guardian & BBC & USA & Wash. \\
\midrule
Guardian & $1.0$ & $0.6$ & $0.6$ & $0.7$ \\
BBC & $1.9$ & $1.6$ & $1.7$ & $0.7$ \\
USA & $1.3$ & $1.2$ & $3.7$ & $2.7$ \\
Wash. & $1.2$ & $1.2$ & $2.0$ & $2.5$ \\
\bottomrule
\end{tabular}
\caption{CIDEr scores of the same captioning model on different train (row) and test (columns) splits. News images and captions from different agencies have different characters, leading to a performance decrease when training set and test set are not from the same agency. }
\label{tab:cross_analysis}
\end{table}

